Urban Outdoor Measurement Study of Phased Antenna Array Impact on Millimeter-Wave Link Opportunities and Beam Misalignment

Exploiting multi-antenna technologies for robust beamsteering to overcome the effects of blockage and beam misalignment is the key to providing seamless multi-Gbps connectivity in millimeter-wave (mm-wave) networks. In this paper, we present the first large-scale outdoor mm-wave measurement study using a phased antenna array in a typical European town. We systematically collect fine-grained 3D angle-of-arrival (AoA) and angle-of-departure (AoD) data, totaling over 50,000 received signal strength measurements. We study the impact of phased antenna arrays in terms of number of link opportunities, achievable data rate and robustness under small-scale mobility, and compare this against reference horn antenna measurements. Our results show a limited number of 2--4 link opportunities per receiver location, indicating that the mm-wave multipath richness in a European town is surprisingly similar to that of dense urban metropolises. The results for the phased antenna array reveal that significant losses in estimated data rate occur for beam misalignments in the order of the half-power beamwidth, with significant and irregular variations for larger misalignments. By contrast, the loss for horn antennas is monotonically increasing with the misalignment. Our results strongly suggest that the effect of non-ideal phased antenna arrays must be explicitly considered in the design of agile beamsteering algorithms.

==> tikz/DROverTXAngles/TRX_TX_EFFECT_MAX_DATARATE_corr.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=220pt,
height=60pt,
at={(0pt,0pt)},
scale only axis,
xmin=-90,
xmax=90,
xlabel near ticks,
xlabel shift={-4pt},
xlabel style={font={\footnotesize\color{black!100}}},
xlabel={$\text{TX antenna beam misalignment from best link (}^\circ\text{)}$},
ymin=0,
ymax=4,
ylabel near ticks,
ylabel shift={-5pt},
ylabel style={font={\footnotesize\color{black!100}}},
ylabel={$T$ (Gbps)},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
%legend style={legend cell align=left, align=left, draw=white!15!black},
ticklabel style={font={\color{black}\footnotesize}},
legend columns=5,
legend style={font={\color{black}\footnotesize}, at={(0.5,1.03)},
anchor=south}
]
\addplot [color=red, thick, densely dashed, mark=o, mark options={solid, red}, mark size=1.2pt]
table[row sep=crcr]{%
-76	2.09665158218931\\
-69	1.5265801057116\\
-60	2.04823878277648\\
-55	0.681570038915382\\
-47	1.54491970997386\\
-42	1.87047380572981\\
-33	1.20560338330928\\
-26	1.57069067880686\\
-20	0.844999920627215\\
-12	1.97428987088665\\
-7	1.36370823351449\\ %66% loss
0	3.99492688965108\\
7	3.33357525867297\\ %17% loss
14	3.45086371211678\\
20	2.55418922698426\\
24	1.54717150907041\\
27	1.51985854458017\\
30	2.73347189459133\\
36	0.798636230625633\\
41	1.46882390218231\\
49	0\\
54	0.974123053376632\\
63	1.86598290871839\\
70	0\\
76	1.26736811125095\\
84	0\\
89	0\\
96	0\\
103	0\\
110	0.72863110424026\\
};
\addlegendentry{1A}

\addplot [color=blue, thick, mark=+, mark options={solid, blue}, mark size=2pt]
  table[row sep=crcr]{%
-76	0\\
-69	0\\
-60	0.696561158385903\\
-55	1.65967218871809\\
-47	1.15556406044262\\
-42	1.09827567621591\\
-33	1.7791506060443\\
-26	1.29526854159605\\
-20	0.859532663976685\\
-12	0.814508417622997\\
-7	1.41931601648163\\ % 60% loss
0	3.53106559421553\\
7	1.61646444098858\\ % 51% loss
14	2.23942728540553\\
20	0.774754950469898\\
24	0.653884808806985\\
27	0\\
30	0.976599146274777\\
36	0.802298927839902\\
41	1.08183836551247\\
49	0\\
54	1.41939200323506\\
63	0\\
70	0\\
76	0\\
84	0\\
89	0\\
96	0\\
103	0\\
110	1.10965422387506\\
};
\addlegendentry{1B}

\addplot [color=green, solid, thick, mark=star, mark options={solid, green}, mark size=2pt]
  table[row sep=crcr]{%
-93	0.682840392519574\\
-86	0\\
-77	0\\
-72	0\\
-64	0.637803262498879\\
-59	1.01398850693723\\
-50	0\\
-43	0.928367741331673\\
-37	1.44959058110542\\
-29	1.19380636986401\\
-24	0.636283860938007\\
-17	0.743229258750359\\
-10	1.20486742922422\\ % 58% loss
-3	2.73616131716494\\
3	2.83519813319267\\
7	1.4325248874025\\ % 49% loss
10	2.17203644941714\\
13	1.31458118331678\\
19	1.22091403245407\\
24	0.623098825947234\\
32	0.908931007369732\\
37	0\\
46	0.776203700985897\\
53	0\\
59	1.18487686186165\\
67	0.807256764168841\\
72	0\\
79	0.903807676929128\\
86	1.32578645846188\\
93	1.10859535439676\\
};
\addlegendentry{1C}

\addplot [color=orange, densely dotted, thick, mark=triangle*, mark options={solid, orange}, mark size=1.2pt]
  table[row sep=crcr]{%
-93	0\\
-86	0\\
-77	0\\
-72	0\\
-64	0\\
-59	0.62168203185241\\
-50	0\\
-43	0\\
-37	0.913735555052071\\
-29	0\\
-24	0\\
-17	0\\
-10	1.58829149703091\\ % 36% loss
-3	2.4807296796608\\
3	2.47036361204881\\
7	0.740051789433112\\ % 70% loss
10	1.63482708664567\\
13	0.654637298448901\\
19	0\\
24	0.59884978749276\\
32	0.758694944674825\\
37	0\\
46	0\\
53	0\\
59	0.618034443224929\\
67	0\\
72	0\\
79	0\\
86	0.806913741533209\\
93	0\\
};
\addlegendentry{2B}

\addplot [color=grey, mark=*, mark options={solid, grey},mark size=1.3pt]
  table[row sep=crcr]{%
-62	0\\
-54	0\\
-49	0\\
-40	1.39003075056137\\
-33	1.14783624834241\\
-27	1.41294621346079\\
-19	0\\
-14	0.846490566529334\\
-7	0.783300478900245\\ % 69%
0	2.55609018478179\\
7	1.57771636945249\\ % 38%
13	1.66145215597833\\
17	0.90567804631877\\
20	1.5488810807461\\
23	0\\
29	0\\
34	0\\
42	0\\
47	0\\
56	0\\
63	0\\
69	0\\
77	0\\
};
\addlegendentry{2D}

\end{axis}
\end{tikzpicture}%


==> tikz/RXElev/Horn_RX_ELEV.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\hspace*{-11pt}
\begin{tikzpicture}

\begin{axis}[%
width=190pt,
height=50pt,
at={(0pt,0pt)},
scale only axis,
unbounded coords=jump,
xmin=-1.8,%-1.3,
xmax=9.6,%8.7,
xlabel near ticks,
xlabel shift={-4pt},
xtick={-0.8,0.2,1.2,2.2,3.2,4.2,5.2,6.2,7.2,8.2},
xticklabels={{-30},{-20},{-10},{0},{10},{20},{30},{40},{50},{60}},
xlabel style={font={\footnotesize\color{black!100}}},
xlabel={$\text{RX elevation angle } \theta_{RX} \text{ (}^\circ\text{)}$},
ymin=0,
ymax=4,
ylabel near ticks,
ylabel shift={-5pt},
ylabel style={font={\footnotesize\color{black!100}}},
ylabel={$T$ (Gbps)},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
ticklabel style={font={\color{black}\footnotesize}},legend style={font={\color{black}\footnotesize}},legend pos=outer north east,
]

\addlegendimage{only marks, mark=o, color=red}
\addlegendentry{1A};
\addlegendimage{only marks, mark=+, color=blue}
\addlegendentry{1B};
\addlegendimage{only marks, mark=asterisk, color=green}
\addlegendentry{1C};


\addplot [color=red, forget plot]
  table[row sep=crcr]{%
0.8	0\\
0.8	1.70926377467911\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
1.8	0\\
1.8	0.90764246442168\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
2.8	0\\
2.8	1.38012233565662\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
3.8	0\\
3.8	0.956307137280659\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
4.8	0\\
4.8	0.612543941867073\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
5.8	0\\
5.8	0.691419108850357\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
6.8	0\\
6.8	0.677019707820117\\
};
\addplot [color=red, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
0.8	0\\
0.8	0.728181362206827\\
};
\addplot [color=red, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
1.8	0.266000032729639\\
1.8	0.675570223458305\\
};
\addplot [color=red, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
2.8	0\\
2.8	0.565119794429375\\
};
\addplot [color=red, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
3.8	0\\
3.8	0.486298309636992\\
};
\addplot [color=red, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
4.8	0\\
4.8	0.342215377373925\\
};
\addplot [color=red, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
5.8	0\\
5.8	0.283846928978584\\
};
\addplot [color=red, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
6.8	0\\
6.8	0.278651637527673\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
0.775	0.394866764328973\\
0.825	0.394866764328973\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
1.775	0.381622311518177\\
1.825	0.381622311518177\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
2.775	0.341894423478104\\
2.825	0.341894423478104\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
3.775	0.301549266626793\\
3.825	0.301549266626793\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
4.775	0\\
4.825	0\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
5.775	0\\
5.825	0\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
6.775	0\\
6.825	0\\
};
\addplot [color=green, draw=none, mark=o, mark options={solid, red}, forget plot]
  table[row sep=crcr]{%
0.8	2.00567094903831\\
0.8	2.12095686243263\\
0.8	2.39717313289876\\
0.8	2.51370788674596\\
0.8	2.58453224605815\\
0.8	2.61749391790811\\
};
\addplot [color=green, draw=none, mark=o, mark options={solid, red}, forget plot]
  table[row sep=crcr]{%
1.8	1.49301181729736\\
1.8	1.61037295477759\\
1.8	1.92382732239294\\
1.8	2.18851226620167\\
1.8	2.44203537173752\\
1.8	2.4629395679676\\
1.8	2.67964378527539\\
1.8	2.93569801904592\\
1.8	2.97634253209338\\
1.8	3.10748973037052\\
1.8	3.16409048346371\\
};
\addplot [color=green, draw=none, mark=o, mark options={solid, red}, forget plot]
  table[row sep=crcr]{%
2.8	1.69096389982617\\
2.8	1.87847049928508\\
2.8	2.50474173608016\\
2.8	2.58767006408599\\
2.8	2.75506607803649\\
2.8	2.83661452876673\\
2.8	3.01372814131339\\
2.8	3.02768496228226\\
2.8	3.12875024183389\\
2.8	3.13302096162348\\
};
\addplot [color=green, draw=none, mark=o, mark options={solid, red}, forget plot]
  table[row sep=crcr]{%
3.8	1.54057767274288\\
3.8	1.7787992419368\\
3.8	1.91134224452556\\
3.8	2.27218484731886\\
3.8	2.35740940902902\\
3.8	2.54415646128542\\
3.8	2.7296007680267\\
3.8	2.82111670695457\\
3.8	2.86640306046521\\
3.8	2.93179687499561\\
};
\addplot [color=green, draw=none, mark=o, mark options={solid, red}, forget plot]
  table[row sep=crcr]{%
4.8	1.06336693489656\\
4.8	1.38638640299493\\
4.8	1.43756046601443\\
4.8	1.6100814908025\\
4.8	1.68496798488868\\
4.8	1.85911998732599\\
4.8	1.8720804527306\\
4.8	1.89326380516799\\
4.8	1.92828831008229\\
4.8	1.94994199828173\\
4.8	1.96341262129056\\
};
\addplot [color=green, draw=none, mark=o, mark options={solid, red}, forget plot]
  table[row sep=crcr]{%
5.8	0.716681921319965\\
5.8	0.723006592234733\\
5.8	0.734391264697418\\
5.8	0.805453196023285\\
};
\addplot [color=green, draw=none, mark=o, mark options={solid, red}, forget plot]
  table[row sep=crcr]{%
6.8	0.746071827173759\\
6.8	0.857300039197486\\
6.8	0.904296502319826\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
1	0\\
1	1.21206095755268\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
2	0\\
2	1.24484286090418\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
3	0\\
3	0.544926315031819\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
4	0\\
4	0\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
5	0\\
5	0\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
6	0\\
6	0\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
7	0\\
7	0\\
};
\addplot [color=blue, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
1	0\\
1	0.556684559633745\\
};
\addplot [color=blue, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
2	0\\
2	0.503883999140395\\
};
\addplot [color=blue, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
3	0\\
3	0.315553856333455\\
};
\addplot [color=blue, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
4	0\\
4	0\\
};
\addplot [color=blue, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
5	0\\
5	0\\
};
\addplot [color=blue, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
6	0\\
6	0\\
};
\addplot [color=blue, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
7	0\\
7	0\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
0.975	0.271862980299043\\
1.025	0.271862980299043\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
1.975	0.312888474213109\\
2.025	0.312888474213109\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
2.975	0\\
3.025	0\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
3.975	0\\
4.025	0\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
4.975	0\\
5.025	0\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
5.975	0\\
6.025	0\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
6.975	0\\
7.025	0\\
};
%\addplot [color=green, draw=none, mark=+, mark options={solid, blue}, forget plot]
%  table[row sep=crcr]{%
%nan	nan\\
%};
%\addplot [color=green, draw=none, mark=+, mark options={solid, blue}, forget plot]
%  table[row sep=crcr]{%
%nan	nan\\
%};
\addplot [color=green, draw=none, mark=+, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
3	0.862120584656047\\
3	0.898216607316604\\
3	1.16089212141095\\
};
\addplot [color=green, draw=none, mark=+, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
4	0.268153317332639\\
4	0.275461186003364\\
4	0.277046672202315\\
4	0.284503973303674\\
4	0.287443107976662\\
4	0.292862643605627\\
4	0.297559133069432\\
4	0.350227578032046\\
4	0.356246522578966\\
4	0.422907054866501\\
4	0.427846718158739\\
4	0.530676606690152\\
};
\addplot [color=green, draw=none, mark=+, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
5	0.272430736553001\\
5	0.277122066762617\\
5	0.279960059866042\\
5	0.2846096299241\\
5	0.284699975564692\\
5	0.336443841793021\\
5	0.341632515792941\\
};
\addplot [color=green, draw=none, mark=+, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
6	0.274776373189305\\
6	0.278201153159154\\
6	0.282037755114332\\
};
\addplot [color=green, draw=none, mark=+, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
7	0.292562905506362\\
7	0.363187491706803\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
-0.8	0\\
-0.8	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
0.2	0\\
0.2	0.660058850022713\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
1.2	0\\
1.2	0.734466928171134\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
2.2	0\\
2.2	0.815938010346046\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
3.2	0\\
3.2	0.697529951066412\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
4.2	0\\
4.2	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
5.2	0\\
5.2	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
6.2	0\\
6.2	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
7.2	0\\
7.2	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
8.2	0\\
8.2	0\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
-0.8	0\\
-0.8	0\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
0.2	0\\
0.2	0.267255845568275\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
1.2	0\\
1.2	0.31875796223613\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
2.2	0\\
2.2	0.336934482215109\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
3.2	0\\
3.2	0.296025141276505\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
4.2	0\\
4.2	0\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
5.2	0\\
5.2	0\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
6.2	0\\
6.2	0\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
7.2	0\\
7.2	0\\
};
\addplot [color=green, line width=4.0pt, forget plot]
  table[row sep=crcr]{%
8.2	0\\
8.2	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
-0.825	0\\
-0.775	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
0.175	0\\
0.225	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
1.175	0\\
1.225	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
2.175	0\\
2.225	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
3.175	0\\
3.225	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
4.175	0\\
4.225	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
5.175	0\\
5.225	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
6.175	0\\
6.225	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
7.175	0\\
7.225	0\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
8.175	0\\
8.225	0\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
-0.8	0.266022895683994\\
-0.8	0.286920590048331\\
-0.8	0.296756726252314\\
-0.8	0.298941961940784\\
-0.8	0.327557193959182\\
-0.8	0.365107593289408\\
-0.8	0.452806214345915\\
-0.8	0.459571553804171\\
-0.8	0.541967679558892\\
-0.8	0.561140749304502\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
0.2	0.683591560218117\\
0.2	0.769858740047928\\
0.2	0.895342219711269\\
0.2	1.04930531173804\\
0.2	1.18723284289655\\
0.2	1.48436357138804\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
1.2	0.927636640449989\\
1.2	1.05337064269526\\
1.2	1.17390522945668\\
1.2	1.44646056951678\\
1.2	1.50398133755171\\
1.2	1.59199381965352\\
1.2	1.74617670876516\\
1.2	1.77747485398643\\
1.2	1.84098627241807\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
2.2	0.921089139943604\\
2.2	0.97311365192333\\
2.2	1.20990438349467\\
2.2	1.34529959318843\\
2.2	1.38367266536588\\
2.2	1.59277276278672\\
2.2	1.61274128789716\\
2.2	1.92941586520441\\
2.2	2.01699612343231\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
3.2	0.905669167489752\\
3.2	0.947592968848752\\
3.2	1.10319893221943\\
3.2	1.34439309622851\\
3.2	1.63929336826553\\
3.2	1.65177505431367\\
3.2	1.66536328577673\\
3.2	1.72045253660511\\
3.2	1.8022694659326\\
3.2	1.92046816608733\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
4.2	0.283388511241763\\
4.2	0.30338656844467\\
4.2	0.30527387863172\\
4.2	0.536952679322213\\
4.2	0.554396558165304\\
4.2	0.604217284270203\\
4.2	0.665953304144941\\
4.2	0.935563779360071\\
4.2	0.947676949153424\\
4.2	1.17381943767683\\
4.2	1.35081839129414\\
4.2	1.38144357654761\\
4.2	1.3943968884719\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
5.2	0.263874182637064\\
5.2	0.277888244374128\\
5.2	0.332869345129599\\
5.2	0.343462336750871\\
5.2	0.351080535688742\\
5.2	0.432840445085692\\
5.2	0.573579521140801\\
5.2	0.713729343571049\\
5.2	0.738958166184107\\
5.2	0.742573108400529\\
5.2	0.7507734924666\\
5.2	0.80929920323045\\
5.2	0.933702159649191\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
6.2	0.274371715436105\\
6.2	0.27900170087206\\
6.2	0.279500673591275\\
6.2	0.295169656926639\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
7.2	0.283612327125949\\
7.2	0.30149380405513\\
7.2	0.302199350279124\\
7.2	0.365012885829453\\
7.2	0.374918362514537\\
7.2	0.409078057067676\\
7.2	0.452192090934317\\
};
\addplot [color=green, draw=none, mark=asterisk, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
8.2	0.26969400456529\\
8.2	0.339041650816823\\
8.2	0.355979310772579\\
8.2	0.377565353083495\\
8.2	0.41368839512511\\
};
\end{axis}
\end{tikzpicture}%

